Laughter Synthesis using Pseudo Phonetic Tokens with a Large-scale In-the-wild Laughter Corpus

We present a large-scale in-the-wild Japanese laughter corpus and a laughter synthesis method. Previous work on laughter synthesis lacks not only data but also proper ways to represent laughter. To solve these problems, we first propose an in-the-wild corpus comprising $3.5$ hours of laughter, which is to our best knowledge the largest laughter corpus designed for laughter synthesis. We then propose pseudo phonetic tokens (PPTs) to represent laughter by a sequence of discrete tokens, which are obtained by training a clustering model on features extracted from laughter by a pretrained self-supervised model. Laughter can then be synthesized by feeding PPTs into a text-to-speech system. We further show PPTs can be used to train a language model for unconditional laughter generation. Results of comprehensive subjective and objective evaluations demonstrate that the proposed method significantly outperforms a baseline method, and can generate natural laughter unconditionally.

==> tables/corpus_comparison.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \caption{Corpus comparison}
    \begin{tabular}{c|ccc}
    Corpus      & \#utterances  & recording & lang. \\ \hline
    Exvo        & xxx           & acted     & En, Zh, Es \\
    OGVC         & xxx           & xxx       & xxx \\
    AudioSet \\
    laughter-net
    \end{tabular}
    \label{tab:corpus_comparison}
\end{table}


self-bleu

==> tables/sub_test.tex <==
\begin{table}[t]
    \centering
    \caption{Results of the subjective evaluations. \textbf{Bold} indicates the best score with $p < 1e-5$ comparing to Baseline.}
    \vspace{1mm}
    %\small
    \begin{tabular}{c|cc}
    \hline
    Model & MOS($\uparrow$) & SMOS($\uparrow$) \\
    \hline\hline
    GT       &     &  NA  \\
    HiFi-GAN & $3.31$  & $4.74$ \\
    \hline 
    Baseline & $1.25$  & $1.20$ \\
    Proposed-L$5$ &  $\mathbf{3.00}$  & $3.07$ \\
    Proposed-L$8$ &  $2.98$  & $3.17$ \\
    Proposed-L$12$ & $2.96$  & $\mathbf{3.22}$ \\
    \hline
    \end{tabular}
    \label{tab:subjective_test}

\end{table}

==> trash.tex <==
\begin{table}[t]
    \centering
    \caption{Results of the objective evaluation of the token language model. \textbf{Bold} indicates the best score with $p < 1e-5$.}
    \vspace{1mm}
    %\small
    \begin{tabular}{c|cc|cc}
    \hline
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{Objective} & \multicolumn{2}{c}{Subjective} \\
     & PPL & Self-BLEU & MOS & SMOS \\
    \hline\hline
    Proposed-L$8$ & $4.67$  &  $89.63$  &   &  \\
    Proposed-L$12$ & $7.57$  & $83.19$  &  &  \\
    \hline
    \end{tabular}
    \label{tab:ulm}
\end{table}

\begin{table}[t]
    \centering
    \caption{Results of the objective evaluation. \textbf{Bold} indicates the best score with $p < 1e-5$ comparing to Baseline.}
    \vspace{1mm}
    %\small
    \begin{tabular}{c|cc}
    \hline
    Model & MCD($\downarrow$) & F0-RMSE($\downarrow$) \\
    \hline\hline
    HiFi-GAN & $6.678$  & $53.704$ \\
    \hline 
    Baseline & $16.593$  & $117.653$ \\
    \makecell[cl]{Baseline w GT feat.} & $10.743$  & $85.689$ \\
    Proposed-L$5$ &  $11.532$  & $\mathbf{80.280}$ \\
    Proposed-L$12$ & $\mathbf{11.406}$  & $81.425$ \\
    \hline
    \end{tabular}
    \label{tab:objective_test}
\end{table}

\begin{table}[t]
    \centering
    \caption{Results of the objective evaluation of the token language model. \textbf{Bold} indicates the best score with $p < 1e-5$.}
    \vspace{1mm}
    %\small
    \begin{tabular}{c|cc|c}
    \hline
    Model & PPL($\downarrow$) & Self-BLEU($\downarrow$) & Self-BLEU (GT)\\
    \hline\hline
    Proposed-L$8$  &  $4.67$ & $89.63$ & $82.41$ \\
    Proposed-L$12$ & $7.57$  & $83.19$ & $62.97$ \\
    \hline
    \end{tabular}
    \label{tab:objective_ulm}
\end{table}
